Clustering Interval-Censored Time-Series for Disease Phenotyping

Unsupervised learning is often used to uncover clusters in data. However, different kinds of noise may impede the discovery of useful patterns from real-world time-series data. In this work, we focus on mitigating the interference of interval censoring in the task of clustering for disease phenotyping. We develop a deep generative, continuous-time model of time-series data that clusters time-series while correcting for censorship time. We provide conditions under which clusters and the amount of delayed entry may be identified from data under a noiseless model. On synthetic data, we demonstrate accurate, stable, and interpretable results that outperform several benchmarks. On real-world clinical datasets of heart failure and Parkinson's disease patients, we study how interval censoring can adversely affect the task of disease phenotyping. Our model corrects for this source of error and recovers known clinical subtypes.

==> header.tex <==
\usepackage[font=normal,format=plain,labelfont=bf,up,textfont=it,up]{caption}
\usepackage{url}
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[swedish,english]{babel}
\usepackage{amssymb, amsmath}
\usepackage{ae}
\usepackage{units}
\usepackage{icomma}
\usepackage{rotating}
\usepackage{natbib}
\usepackage[usenames, dvipsnames]{color}
\usepackage{graphicx}
\usepackage{bbm}
\usepackage{algorithmic}
\usepackage{listings}
\usepackage{cite}
\usepackage{todonotes}
\usepackage{subcaption}
\usepackage{enumerate}
%\usepackage{natbib}
\usepackage{marginnote}
\usepackage{titling}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{fullpage}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{comment}
\usepackage{afterpage}
\usepackage{amsmath,comment}
\usepackage{tikz-qtree}
\usepackage{tikz}
\usepackage[draft]{fixme}
\fxsetup{inline,nomargin,theme=color}
\newtheorem{thmlem}{Lemma}
\newtheorem{thmcol}{Corollary}
\newtheorem{thmprop}{Proposition}
\newtheorem{thmthm}{Theorem}
\newtheorem{thmappthm}{Theorem}
\newtheorem{thmasmp}{Assumption}
\newtheorem{thmcorr}{Corollary}

\newtheorem{thmappasmp}{Assumption}
\renewcommand{\thethmappasmp}{A\arabic{thmappasmp}}
\newtheorem{thmapplem}{Lemma}
\renewcommand{\thethmapplem}{A\arabic{thmapplem}}
\newtheorem{thmappcol}{Corollary}
\renewcommand{\thethmappcol}{A\arabic{thmappcol}}

\theoremstyle{definition}
\newtheorem{thmdef}{Definition}

\newtheorem{thmappdef}{Definition}
\renewcommand{\thethmappdef}{A\arabic{thmappdef}}



\newenvironment{thmproof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\textit{#1.}}]}{\end{trivlist}}
\newenvironment{thmproofsketch}[1][Proof sketch]{\begin{trivlist}
\item[\hskip \labelsep {\textit{#1.}}]}{\end{trivlist}}
\newtheorem{proposition}{Proposition}

\def\bff{\boldsymbol{f}}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bE{\mathbf{E}}
\def\bw{\mathbf{w}}
\def\cP{\mathcal{P}}
\def\bv{\mathbf{v}}
\def\hbu{\hat{\bu}}
\def\hbv{\hat{\bv}}
\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bmu{\boldsymbol{\mu}}
\def\bgamma{\boldsymbol{\gamma}}
\def\bdelta{\boldsymbol{\delta}}
\def\E{\mathbb{E}}
\def\cN{\mathcal{N}}
\def\cL{\mathcal L}
\def\cD{\mathcal D}
\def\cC{\mathcal C}
\def\cT{\mathcal T}
\def\cX{\mathcal X}
\def\cY{\mathcal Y}
\def\cH{\mathcal H}
\def\cU{\mathcal U}
\def\cS{\mathcal S}
\def\cZ{\mathcal Z}
\def\cF{\mathrm{G}}
\def\cFL{\mathrm{F}_{Lip(1)}}
\def\cx{\mathcal x}
\def\cR{\mathcal{R}}
\def \R{\mathbb{R}}
\def \pFr {p^{F}_\Phi(r,t)}
\def \pCr {p^{CF}_\Phi(r,t)}
\def \epehe{\epsilon_{\text{PEHE}}}
\def \eate{\epsilon_{\text{ATE}}}
\def \eatt{\epsilon_{\text{ATT}}}
\def \eclass{\epsilon_{\text{Class}}}
\def \epehenn{{\epehe}_{nn}}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\pc}{p^{t=0}}
\newcommand{\pt}{p^{t=1}}
\newcommand{\ptr}{•}
\newcommand{\dPhi}{\frac{\partial \Phi(x)}{\partial x}}
\newcommand{\dPsi}{\frac{\partial \Psi(r)}{\partial r}}

%\newcommand{\errTC}{\mathbb{E}_T \left[\text{err}_{\Phi,h}(C)\right]}
%\newcommand{\errTT}{\mathbb{E}_T \left[\text{err}_{\Phi,h}(T)\right]}
%\newcommand{\errCC}{\mathbb{E}_C \left[\text{err}_{\Phi,h}(C)\right]}
%\newcommand{\errCT}{\mathbb{E}_C \left[\text{err}_{\Phi,h}(T)\right]}

\newcommand{\errTC}{\mathbb{E}_T \left[\text{err}_C(\Phi,h)\right]}
\newcommand{\errTT}{\mathbb{E}_T \left[\text{err}_T(\Phi,h)\right]}
\newcommand{\errCC}{\mathbb{E}_C \left[\text{err}_C(\Phi,h)\right]}
\newcommand{\errCT}{\mathbb{E}_C \left[\text{err}_T(\Phi,h)\right]}

\newcommand{\lyth}{\ell_{h,\Phi}(x,t)}
\newcommand{\lythr}{\ell_{h,\Phi}(\Psi(r),t)}
\newcommand{\lyxzeroh}{\ell_{h,\Phi}(x,0)}
\newcommand{\lyxoneh}{\ell_{h,\Phi}(x,1)}
\newcommand{\lyzeroh}{\ell_{h,\Phi}(r,0)}
\newcommand{\lyoneh}{\ell_{h,\Phi}(r,1)}
\newcommand{\lyzerohpsi}{\ell_{h,\Phi}(\Psi(r),0)}
\newcommand{\lyonehpsi}{\ell_{h,\Phi}(\Psi(r),1)}

\newcommand{\Jphix}{\frac{\partial \Phi (x)}{\partial x}}
\newcommand{\GP}{\Gamma_\Phi}
\def\mmd{\mbox{\sc mmd}}
\def\diag{\mbox{diag}}

\DeclareMathOperator*{\disc}{disc}
\DeclareMathOperator*{\expect}{E}

\def\transu{\Delta\bu}
\def\transv{\Delta\bv}
\def\pr{\mbox{Pr}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\setlength{\parskip}{\baselineskip}
\setlength{\parindent}{0pt}


==> identifiability_proof_1.tex <==


\begin{algorithm}[t]
   \caption{Procedure for the identification of model parameters}\label{alg:identifiability}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Visit times $X \in \mathbb{R}^{N \times M}$, biomarkers $Y \in \mathbb{R}^{N \times M \times J}$, polynomial degree $P$, invertible function $f$
    \STATE{\bfseries Output:} $\theta^P$, $\delta_1,\ldots,\delta_N$, $s_1,\ldots,s_N$ for each patient
    \STATE \textbf{Step 1: Transform the observed biomarkers;} $\tilde{Y}=f^{-1}(Y)$
    \STATE \textbf{Step 2: Obtain time-shifts using a single biomarker;}
    \STATE a) Shift all observations of the first biomarker to obtain: $Q = \tilde{Y}[:,:,1]-\max \tilde{Y}[:,:,1]$
    \STATE b) For each patient $i$, estimate the parameters $\tilde{\theta^1}_i$ of $\kappa(x;\tilde{\theta^1}_i)$ using $((x_i^1,q_i^1),\ldots,(x_i^M,q_i^M)$ via polynomial regression, 
    \STATE c) Compute upto $P$ real roots of polynomial $\kappa(x, \tilde{\theta^1}_i)$ for each patient $i$ as $R_i=\{r_1,\ldots,r_P\}$ and set $\gamma_i=\min R_i$
    \STATE d) Re-estimate $\tilde{\theta^1}_i$ using $((x_i^1-\gamma_i,q_i^1),\ldots,(x_i^M-\gamma_i,q_i^M)$ via polynomial regression,
    \STATE e) Cluster $\tilde{\theta^j}_i$ across patients via K-means clustering to yield cluster identities $s_1,\ldots,s_N$
    \STATE f) $\forall k\;\; \eta_k = \min \{\gamma_i|i \text{ s.t. } s_i=k\}$ and $\delta_i = \gamma_i-\eta_{s_i}$
    \STATE \textbf{Step 3: Re-estimate polynomial coefficients using shifted observation times;}
    \FOR{biomarker $j=1$ {\bfseries to} $J$}
    \STATE For each patient, estimate the parameters $\theta^j_i$ of $\kappa(x;\hat{\theta^j}_i)$ using $((x_1^1-\delta_i,y_1^1[j]),\ldots,(x_1^M-\delta_i,y_1^M[j])$ via polynomial regression, 
    \ENDFOR
    \STATE Return $\theta^P=[\theta^1|\ldots|\theta^J],\{\delta_1,\ldots, \delta_N\},\{s_1,\ldots, s_N\}$
\end{algorithmic}
\end{algorithm}

We provide the proof for Theorem \ref{thm:identifiability} below: 

\begin{proof}
The proof is constructive; i.e. we give an algorithm for the identification of the parameters of the model in Equation \ref{eqn:identifiable_model}. 
The algorithm for identification is presented in Algorithm \ref{alg:identifiability} and proceeds in three steps.

\textbf{Step 1:} The first step transforms the observed biomarkers by applying the inverse of function $f$, which exists by Assumption \ref{assum:functionals}. This leaves us with data as: $$f^{-1}(y_i^m) = \kappa(x_i^m + \delta_i; \theta^P_{s_i})\; \;\forall i \in N, m \in M$$
i.e. for all bio-markers, across all patients, we have observations from different polynomial functions. 

\textbf{Step 2:} Without loss of generality, this step uses the first biomarker to identify the values of $\delta_i$ for each patient. 

\begin{itemize}
    \item a) If $P$ is odd, we are guaranteed to find at least one root. If $P$ is even, the polynomial may have zero roots. Therefore, we shift the observations down by the largest value observed among all the data. This guarantees that the resulting polynomial coefficients estimated from data all have at least one real root.
    \item b) Next, we estimate the polynomial coefficients for each patient separately; we are guaranteed recovery by Assumption \ref{assum:enough_obs}. 
    \item c) We solve to find the roots for each polynomial and define $\gamma_{i}$ as the smallest root of the polynomial
    \item d) Next, we shift the observational time-staps by $\gamma_i$, this operation \emph{centers} all the polynomials at the origin and we re-estimate the coefficients of each \emph{shifted} polynomial
    \item e) We cluster the coefficients estimated in step (d). By construction, we know that $s_i = s_{i'}\iff \theta_i = \theta_{i'}$ which guarantees that clustering recovers the true-underlying subtype for each patient. 
    \item f) Finally we stratify patients by their subtype, and we define $\delta_i$ as the difference between their smallest root and the smallest value of $\gamma_i$ among all other patients within that subtype. By Assumption \ref{assum:delta0}, we know that for each subtype, there exists a patient for whom $\delta_i=0$, this reference patient will also be the one whose polynomial has the smallest root. Therefore, by shifting each patient's smallest root by their reference patient's smallest root, we can recover the original time-shifts. 
\end{itemize}
\textbf{Step 3:} Given the values of $\delta_1,\ldots,\delta_N$ from Step 2, we can now estimate the true values of the polynomial coefficients exactly in the noiseless setting via polynomial regression. 
\end{proof}


==> learning.tex <==
\subsection{Step $1$: Learning}
We learn the parameters $\gamma$ of the model in Equation \ref{eqn:gen_process} via maximum likelihood estimation. 
Since the model is a non-linear latent variable model, we maximize a variational lower bound on the conditional likelihood of data given observation time-stamps.
% (derived for a single patient's sequence). 
%\begin{align}
%\label{eqn:lw_bd}
%    \log p(Y|X;\gamma) \geq \mathbb{E}_{q(Z|X,Y;\phi)}\left[ \log\frac{p(Y,Z,\delta|X,\delta;\gamma)}{q(Z|X,Y;\phi)}\right] %+ \underbrace{\int_{\delta} q(\delta)  \log\frac{p(\delta)}{q(\delta)}}_{\text{constant wrt $\gamma,\phi$}}
%\end{align}
We parameterize a variational distribution for $Z$ via an inference network \citep{kingma2013auto,rezende2014stochastic} with parameters $\phi$; and can derive a lower bound for a patient as:
\begin{align}
%    &\log p(Y|X) \geq \mathcal{L}(Y|X;\gamma,\phi)\nonumber \\ 
\log p(Y|X;\gamma) \geq \mathcal{L}(Y|X;\gamma,\phi) =  \mathbb{E}_{q(Z|X,Y;\phi)}\Big[& \log \sum_{\delta} p(Y|X,\delta,Z;\gamma) p(\delta) + \log \frac{p(Z)}{q(Z|X,Y;\phi)}\Big]
\label{eqn:var_lwbd}
\end{align}
We refer the reader to the appendix for the proof of the same.
Equation \ref{eqn:var_lwbd} is differentiable in $\gamma,\phi$ using the re-parameterization trick~\cite{kingma2013auto, rezende2014stochastic} for the outer expectation and 
the log-sum-exp trick for the inner sum. A natural next step would be to learn via gradient ascent on the objective function with $\max_{\gamma, \phi} \sum_{i=1}^{N}\mathcal{L}(Y_i|X_i;\gamma,\phi)$. 
However, we found this approach unstable, often getting stuck in poor local optima.
Instead, we note that for all values of $\hat{\delta}$:
\begin{align}
\mathcal{L}(Y|X;\gamma,\phi)&>\mathcal{L}(Y|X;\gamma,\phi,\hat{\delta}) =  \mathbb{E}_{q(Z|X,Y;\phi)}\Big[\log p(Y|X,\hat{\delta},Z;\gamma) p(\hat{\delta}) + \log \frac{p(Z)}{q(Z|X,Y;\phi)}\Big]
\label{eqn:var_lwbd_delta}
\end{align}
We then learn via subgradient ascent: $\max_{\gamma, \phi} \sum_{i=1}^{N} \max_{\hat{\delta}\in \mathcal{D}}\mathcal{L}(Y_i|X_i;\gamma,\phi,\hat{\delta}_i)$
% \label{eqn:subgradient}
where we first obtain $\hat{\delta}_i = \arg\max_{\delta\in \mathcal{D}} \mathcal{L}(Y_i | X_i;\gamma,\phi,\delta)$ and 
use this to 
derive gradients $\nabla_{\gamma,\phi} \mathcal{L}(Y_i | X_i;\gamma,\phi,\hat{\delta}_i)$. 
One can view our approach as leveraging Maximum-A-Posteriori inference for $\delta$
nested within a variational approach for $Z$. Given our choice to use a discretized $\delta$ that lies within a tractable, finite set, we found this choice to work well and can be made more efficient if necessary, e.g.  practitioners can trivially parallelize the search over $\hat{\delta}_i$.
%An alternative learning algorithm could parameterize a variational distribution over both $\delta$ and $Z$.

% We detail how we select $D, \delta^-,$ and $\delta^+$ in Section~\ref{sec:hyperparameters}.  %$\delta^+$ is chosen dynamically per patient.
%A subgradient is obtained by finding $$ and then computing .
%
%To do gradient based learning, we need to be able to approximate
%the inner and outer expectation. 

The expectation in Equation \ref{eqn:var_lwbd} 
is identical to the variational lower bound
used in learning variational autoencoders \cite{kingma2013auto}
and is amenable to gradient based learning via stochastic
backpropagation. In practice, we use a recurrent neural
network (RNN) to parameterize the inference network.  
We concatenate the observation times $X$ and clinical biomarkers $Y$ as inputs into the RNN with parameters $\phi_1$. We use the last hidden state of the RNN, $h$, to parameterize $q(Z|X,Y)= \mathcal{N}(\mu(h;\phi_2), \Sigma(h;\phi_3))$ with $\mu$ and $\Sigma$ parameterized as neural networks with parameters $\phi_2$ and $\phi_3$, respectively. The parameters of the inference network are the set $\phi=\{\phi_1,\phi_2,\phi_3\}$. 

%Equation \ref{eqn:var_lwbd_delta} could be an equality if all elements inside the sum over $\delta$ in Equation \ref{eqn:var_lwbd} are the same. This, however, would imply that $\delta$ has no effect on the conditional likelihood of the data, which is impossible by construction.

% \textbf{Sublign-MoG} In Eq.~\ref{eqn:gen_process}, we assume a uniform normal prior for the latent variable $z_i$. 
% One potential modification to the model presented would be to allow for a more flexible prior using a mixture of Gaussians ~\cite{tomczak2018vae}. Let $L$ denote the number of mixture components, then, we may assume $z_i\sim\sum_{l=1}^L\pi_l\mathcal{N}(\mu_l;\Sigma_l)$. We will study this model as SubLign-MoG.

% \textbf{Sublign:} We introduced maximum likelihood estimation of a generative model (Eq. \ref{eqn:var_lwbd}) using approximate Bayesian inference. When the model is used in conjunction with an inference network it is referred to as a variational autoencoder. From the perspective of learning autoencoders, the second term in 
% Eq. ~\ref{eqn:var_lwbd} provides a regularizing effect to ensure that the approximate posterior remains close to the prior
% distribution. 
% However, should we wish to forgo the interpretation of the model as a generative model that we can sample from, then, we open up new possibilities for different learning algorithms. For example, during training we may tune the learning algorithm using parameter $\beta$:
% \begin{align}
% \mathcal{L}_{\beta}(Y_i |& X_i;\gamma,\phi,\hat{\delta}_i) \nonumber \\
% &=\mathbb{E}_{q(Z|X,Y;\phi)}\Big[\log p(Y|X,\hat{\delta},Z;\gamma)p(\hat{\delta}) \nonumber \\
% &\quad \quad + \beta \log \frac{p(Z)}{q(Z|X,Y;\phi)}\Big]
% \label{eqn:beta_vae}
% \end{align}
% While $\beta$ can be $> 1$, as studied in~\cite{higgins2017beta}, we consider the case where $\beta \in [0,1]$, similar to~\cite{liang2018variational}. Note that $\beta=1$ corresponds to the traditional variational autoencoder~\cite{kingma2013auto}. 
